Physics-Informed Regularization for Domain-Agnostic Dynamical System Modeling

Learning complex physical dynamics purely from data is challenging due to the intrinsic properties of systems to be satisfied. Incorporating physics-informed priors, such as in Hamiltonian Neural Networks (HNNs), achieves high-precision modeling for energy-conservative systems. However, real-world systems often deviate from strict energy conservation and follow different physical priors. To address this, we present a framework that achieves high-precision modeling for a wide range of dynamical systems from the numerical aspect, by enforcing Time-Reversal Symmetry (TRS) via a novel regularization term. It helps preserve energies for conservative systems while serving as a strong inductive bias for non-conservative, reversible systems. While TRS is a domain-specific physical prior, we present the first theoretical proof that TRS loss can universally improve modeling accuracy by minimizing higher-order Taylor terms in ODE integration, which is numerically beneficial to various systems regardless of their properties, even for irreversible systems. By integrating the TRS loss within neural ordinary differential equation models, the proposed model TREAT demonstrates superior performance on diverse physical systems. It achieves a significant 11.5% MSE improvement in a challenging chaotic triple-pendulum scenario, underscoring TREAT's broad applicability and effectiveness.

==> section/implementation.tex <==
\textbf{TANGO}
\par
Our implementation of TANGO follows \citep{LGODE}. We implement the initial state encoder using a 2-layer GNN with observation representation dimension of 64 across all datasets. We use ReLU for nonlinear activation. For the self-attention module, we set the output dimension to 128. The encoder's output dimension is set to 16, and we add 64 additional dimension to the output of the recognition model to stabilize the training process. The GraphODE generative model is implemented with a single-layer GNN with hidden dimension 128. To compute trajectories, we use the Runge-Kutta method from torchdiffeq python package \cite{chen2021eventfn} as the ODE solver, and a one-layer MLP as the decoder.

We implement our model in pytorch. Encoder, generative model and the decoder parameters are jointly optimized with AdamW optimizer \cite{loshchilov2017decoupled}. \ji{todo: add details} with learning rate 0.0005. Batch size for simulated datsests are set as 256.

\textbf{LatentODE}
\par
We implement the Latent ODE sequence to sequence model as specified in \cite. We use a 4-layer ODE function in the recognition ODE, and a 2-layer ODE function in the generative ODE. The recognition and generative ODE use Euler and Dopri5 as solvers \cite, respectively. The number of units per layer is 1000 in the ODE functions, and 50 in GRU update networks. The dimension of the recognition model is set to 100.  The model is trained with a learning rate of 0.001 with an exponential decay rate of 0.999 across different experiments. Note that since latentODE is a single-agent model, we compute the trajectory of each object independently when applying it to multi-agent systems.

\textbf{HODEN}
\par
To adapt HODEN, which requires full initial states of all objects, to systems with partial observations, we compute each object’s initial state via linear spline interpolation if it is missing. Following the setup in \cite, we use two 2-layer linear networks with Tanh activation in between as the ODE functions for a state and the rate of change of a state. Each network has a 1000-unit layer followed by a single unit layer.The model is trained with a learning rate of 0.00001 using a cosine scheduler.

\textbf{TRSODEN}
\par
Similar to HODEN, we compute each object’s initial state via linear spline interpolation if it is missing. As in \cite, we use a 2-layer linear network with Tanh activation in between as the ODE functions, and the Leapfrog solver \cite. The network has 1000 hidden units, and is trained with a learning rate of 0.00001 using a cosine scheduler.

==> section/relatedwork.tex <==
\section{Related Work}
\textbf{Neural Simulators for Multi-agent Dynamical Systems.}
Building a neural simulator that can understand and predict multi-agent system dynamics from observational data has attracted lots of attention.
Graph Neural Networks (GNNs) achieve the state-of-art performance which approximates pair-wise node (agent) interaction through message passing to impose strong spatial inductive bias. The majority of them are discrete models, which learn a fixed-step state transition function such as to predict trajectories from timestamp t to timestamp t+1. Despite their superior performance, discrete GNN models~\citep{IN,NRI,learn_to_simulate} have two main limitations: (1) they are not able to adequately model systems that are continuous in nature such as n-body systems. (2) they cannot deal with irregular-observed systems, where the observations for different agents are not temporally aligned and can happen at arbitrary time intervals. 
In contrast, neural ordinary differential equation (ODE) methods are continuous models that are superior to model system dynamics in the long-range and with irregular observations. Specifically, they employ GNN as the ODE function to model continuous system dynamics in the latent space,  with an encoder that infers latent initial states of nodes from historical data. These models are known as GraphODEs~\citep{LGODE,hope,ndcn}, which show superior generalization ability and efficiency in making long-range predictions.


\textbf{Physics-informed Neural Networks.}
Injecting physical inductive bias helps neural simulators to be trained more data efficiently and make more accurate predictions. Popular properties include 1.) \textit{Spatial Invariance}, \ie models should be invariant under geometric translation/rotation~\cite{e3gnn,keriven2019universal}; 2.) \textit{Energy conservation}~\cite{hamiltonianNN}, which preserves the total energies for the system over time. 
Towards the second category, not all systems are strictly energy-conservative. For non-isolated systems that have interactions with the environments, pure data-driven approaches may result in system energy changing sharply, which is unrealistic. We therefore would like to build a general-purpose model that can prevent such abrupt energy changes, so as to have the flexibility to cover both conservative and non-conservative dynamical systems.
One prior work also injects time-reversal symmetry into neural networks~\cite{trsode}. However, they cannot model multi-agent interactions and work only for fully-observable systems (with initial states as model input), while our method based on GraphODE is well suited for modelling multi-agent and irregularly observed system. We also theoretically connect time-reversal symmetry loss to how it helps to reduce numerical error. We also illustrate our implementation to achieve time-reversal symmetry has a lower error bound compared to their implementation. 







